Encoding Compositionality in Classical Planning Solutions

Classical AI planners provide solutions to planning problems in the form of long and opaque text outputs. To aid in the understanding transferability of planning solutions, it is necessary to have a rich and comprehensible representation for both human and computers beyond the current line-by-line text notation. In particular, it is desirable to encode the trace of literals throughout the plan to capture the dependencies between actions selected. The approach of this paper is to view the actions as maps between literals and the selected plan as a composition of those maps. The mathematical theory, called category theory, provides the relevant structures for capturing maps, their compositions, and maps between compositions. We employ this theory to propose an algorithm agnostic, model-based representation for domains, problems, and plans expressed in the commonly used planning description language, PDDL. This category theoretic representation is accompanied by a graphical syntax in addition to a linear notation, similar to algebraic expressions, that can be used to infer literals used at every step of the plan. This provides the appropriate constructive abstraction and facilitates comprehension for human operators. In this paper, we demonstrate this on a plan within the Blocksworld domain.

==> figures/algorithm.tex <==
\begin{algorithm}[H]
\textbf{Input:} solution, problem, domain\;
\textbf{Output:} StringDiagram\;
 n\_steps := length(solution)\;
 init\_slice := MakeSlice(problem["init"], domain["predicates"])\;
 goal\_slice := MakeSlice(problem["goal"], domain["predicates"])\;
 \\
 \tcp{Backward Pass}
 \For{$i := \text{n\_steps}:-1:-2$}{
    curr\_slice := goal\;
  \eIf{i $<$ 0}{
   above\_morphism := init\;
   }{
   above\_morphism := solution[i]\;
  }
  above\_strings := MakeStrings(above\_morphism["codomain"])\;
  above\_slice := []\;
  \For{$m := curr\_slice$}{
      \eIf{typeof(m) == IdentityMorphism}{
        s := m["domain"]\;
          \eIf{s in above\_strings}{
          above\_strings.remove(s)
          }{
          above\_slice.push(s)
          }
      }{
        s := m["domain"]
        \For{s}{
        \eIf{s in above\_strings}{
          above\_strings.remove(s)
          }{
          above\_slice.push(s)
          }
        }
      }
  }
 }
 \caption{Autoweave String Diagram}
\end{algorithm}
\caption{To make a PDDL solution, domain, or problem element a slice means to convert actions to morphisms and standalone predicates to identity morphisms and collection them in an ordered list, indicated by \texttt{MakeSlice}. To convert a slice to \textit{strings} requires you choose domain or codomain and convert those objects into a list of identity morphisms preserving order, indicated by \texttt{MakeStrings}.}

==> figures/blocks_domain.tex <==
\begin{verbatim}
(define (domain BLOCKS)
  (:requirements :strips)
  (:predicates (on ?x ?y)
	       (ontable ?x)
	       (clear ?x)
	       (handempty)
	       (holding ?x)
	       )
  (:action pick-up
	     :parameters (?x)
	     :precondition (and (clear ?x) (ontable ?x) (handempty))
	     :effect
	     (and (not (ontable ?x))
		   (not (clear ?x))
		   (not (handempty))
		   (holding ?x)))
  (:action put-down
	     :parameters (?x)
	     :precondition (holding ?x)
	     :effect
	     (and (not (holding ?x))
		   (clear ?x)
		   (handempty)
		   (ontable ?x)))
  (:action stack
	     :parameters (?x ?y)
	     :precondition (and (holding ?x) (clear ?y))
	     :effect
	     (and (not (holding ?x))
		   (not (clear ?y))
		   (clear ?x)
		   (handempty)
		   (on ?x ?y)))
  (:action unstack
	     :parameters (?x ?y)
	     :precondition (and (on ?x ?y) (clear ?x) (handempty))
	     :effect
	     (and (holding ?x)
		   (clear ?y)
		   (not (clear ?x))
		   (not (handempty))
		   (not (on ?x ?y)))))
\end{verbatim}

==> figures/blocks_exp.tex <==
\left(\mathrm{id}_{clear c} \otimes \mathrm{id}_{ontable c} \otimes \mathrm{id}_{clear b} \otimes \mathrm{id}_{ontable b} \otimes \mathrm{id}_{\mathrm{handempty}} \otimes \mathrm{id}_{clear a}\right) 

\cdot

\left(\mathrm{id}_{clear c} \otimes \mathrm{id}_{ontable c} \otimes \mathrm{id}_{clear b} \otimes \mathrm{id}_{ontable b} \otimes \mathrm{id}_{\mathrm{handempty}} \otimes
\mathrm{id}_{clear a}\right) 

\cdot 

\left(\mathrm{id}_{clear c} \otimes \mathrm{id}_{ontable c} \otimes pick-up \otimes \mathrm{id}_{clear a}\right) 

\cdot 

\left(\mathrm{id}_{clear c} \otimes \mathrm{id}_{ontable c} \otimes \mathrm{id}_{holding b} \otimes \mathrm{id}_{\neg ontable b} \otimes \mathrm{id}_{\neg clear b} \otimes \sigma_{\neg handempty,clear a}\right) 

\cdot 

\left(\mathrm{id}_{clear c} \otimes \mathrm{id}_{ontable c} \otimes \mathrm{id}_{holding b} \otimes \mathrm{id}_{\neg ontable b} \otimes \sigma_{\neg clear b,clear a} \otimes \mathrm{id}_{\neg handempty}\right) 

\cdot 

\left(\mathrm{id}_{clear c} \otimes \mathrm{id}_{ontable c} \otimes \mathrm{id}_{holding b} \otimes \sigma_{\neg ontable b,clear a} \otimes \mathrm{id}_{\neg clear b} \otimes \mathrm{id}_{\neg handempty}\right) 

\cdot 

\left(\mathrm{id}_{clear c} \otimes \mathrm{id}_{ontable c} \otimes \mathrm{stack} \otimes \mathrm{id}_{\neg ontable b} \otimes \mathrm{id}_{\neg clear b} \otimes \mathrm{id}_{\neg handempty}\right) 

\cdot 

\left(\mathrm{id}_{clear c} \otimes \mathrm{id}_{ontable c} \otimes \sigma_{clear b,\mathrm{handempty}} \otimes \mathrm{id}_{on b a} \otimes \mathrm{id}_{\neg holding b} \otimes \mathrm{id}_{\neg clear a} \otimes \mathrm{id}_{\neg ontable b} \otimes \mathrm{id}_{\neg clear b} \otimes \mathrm{id}_{\neg handempty}\right) 

\cdot 

\left(pick-up \otimes \mathrm{id}_{clear b} \otimes \mathrm{id}_{on b a} \otimes \mathrm{id}_{\neg holding b} \otimes \mathrm{id}_{\neg clear a} \otimes \mathrm{id}_{\neg ontable b} \otimes \mathrm{id}_{\neg clear b} \otimes \mathrm{id}_{\neg handempty}\right) 

\cdot 

\left(\mathrm{id}_{holding c} \otimes \mathrm{id}_{\neg ontable c} \otimes \mathrm{id}_{\neg clear c} \otimes \sigma_{\neg handempty,clear b} \otimes \mathrm{id}_{on b a} \otimes \mathrm{id}_{\neg holding b} \otimes \mathrm{id}_{\neg clear a} \otimes \mathrm{id}_{\neg ontable b} \otimes \mathrm{id}_{\neg clear b} \otimes \mathrm{id}_{\neg handempty}\right) 

\cdot 

\left(\mathrm{id}_{holding c} \otimes \mathrm{id}_{\neg ontable c} \otimes \sigma_{\neg clear c,clear b} \otimes \mathrm{id}_{\neg handempty} \otimes \mathrm{id}_{on b a} \otimes \mathrm{id}_{\neg holding b} \otimes \mathrm{id}_{\neg clear a} \otimes \mathrm{id}_{\neg ontable b} \otimes \mathrm{id}_{\neg clear b} \otimes \mathrm{id}_{\neg handempty}\right) 

\cdot 

\left(\mathrm{id}_{holding c} \otimes \sigma_{\neg ontable c,clear b} \otimes \mathrm{id}_{\neg clear c} \otimes \mathrm{id}_{\neg handempty} \otimes \mathrm{id}_{on b a} \otimes \mathrm{id}_{\neg holding b} \otimes \mathrm{id}_{\neg clear a} \otimes \mathrm{id}_{\neg ontable b} \otimes \mathrm{id}_{\neg clear b} \otimes \mathrm{id}_{\neg handempty}\right) 

\cdot 

\left(\mathrm{stack} \otimes \mathrm{id}_{\neg ontable c} \otimes \mathrm{id}_{\neg clear c} \otimes \mathrm{id}_{\neg handempty} \otimes \mathrm{id}_{on b a} \otimes \mathrm{id}_{\neg holding b} \otimes \mathrm{id}_{\neg clear a} \otimes \mathrm{id}_{\neg ontable b} \otimes \mathrm{id}_{\neg clear b} \otimes \mathrm{id}_{\neg handempty}\right) 

% : clear c \otimes ontable c \otimes clear b \otimes ontable b \otimes \mathrm{handempty} \otimes clear a \to clear c \otimes \mathrm{handempty} \otimes on c b \otimes \neg holding c \otimes \neg clear b \otimes \neg ontable c \otimes \neg clear c \otimes \neg handempty \otimes on b a \otimes \neg holding b \otimes \neg clear a \otimes \neg ontable b \otimes \neg clear b \otimes \neg handempty

==> figures/blocks_plan.tex <==
\begin{verbatim}
pick-up b
stack b a
pick-up c
stack c b
\end{verbatim}

==> figures/blocks_problem.tex <==
\begin{verbatim}
(define (problem BLOCKS-3-0)
    (:domain BLOCKS)
    (:objects a b c)
    (:init (clear c) (clear a) (clear b) 
            (ontable c) (ontable a) 
            (ontable b) (handempty))
    (:goal (AND (on c b) (on b a)))
)
\end{verbatim}

==> figures/resource_table.tex <==
\begin{table*}[]
\begin{tabular}{lllllllllllllllllllll}
Step & Action & \multicolumn{19}{l}{Available predicates} \\
Start &  & clear c &  & ontable c &  & clear b &  & ontable b &  & handempty &  & clear a &  & ontable a ?? &  &  &  &  &  &  \\
Step 1 & pick-up & clear c &  & ontable c &  &  &  &  &  &  &  & clear a &  &  &  &  & holding b &  &  &  \\
Step 2 & stack & clear c &  & ontable c &  &  & $\neg$clear b &  & $\neg$ontable b &  & $\neg$handempty &  &  &  &  &  &  &  &  &  \\
Step 3 & pick-up &  &  &  &  & clear b & $\neg$clear b &  & $\neg$ontable b &  & $\neg$handempty &  & $\neg$clear a &  & on b a &  &  & $\neg$holding b & holding c &  \\
Step 4 & stack &  & $\neg$clear c &  & $\neg$ontable c &  & $\neg$clear b &  & $\neg$ontable b &  & $\neg$handempty &  & $\neg$clear a &  & on b a &  &  & $\neg$holding b &  &  \\
End &  & clear c & $\neg$clear c &  & $\neg$ontable c &  & $\neg$clear b &  & $\neg$ontable b & handempty & $\neg$handempty &  & $\neg$clear a &  & on b a & on c b &  & $\neg$holding b &  & $\neg$holding c
\end{tabular}
\end{table*}

==> figures/resource_table_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{tabular}{|
>{\columncolor[HTML]{EFEFEF}}l |llllllllllllllllllll}
\hline
\textbf{Step} & \cellcolor[HTML]{EFEFEF}\textbf{Action} & \multicolumn{19}{l}{\cellcolor[HTML]{EFEFEF}\textbf{Available predicates}} \\ \hline
\textbf{Start} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{clear c} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{ontable c} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{clear b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{ontable b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{handempty} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{clear a} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{ontable a ??} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\textbf{Step 1} & \multicolumn{1}{l|}{pick-up} & \multicolumn{1}{l|}{clear c} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{ontable c} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{clear a} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{holding b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\textbf{Step 2} & \multicolumn{1}{l|}{stack} & \multicolumn{1}{l|}{clear c} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{ontable c} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$clear b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$ontable b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$handempty} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\textbf{Step 3} & \multicolumn{1}{l|}{pick-up} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{clear b} & \multicolumn{1}{l|}{$\neg$clear b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$ontable b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$handempty} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$clear a} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{on b a} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$holding b} & \multicolumn{1}{l|}{holding c} & \multicolumn{1}{l|}{} \\ \hline
\textbf{Step 4} & \multicolumn{1}{l|}{stack} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$clear c} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$ontable c} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$clear b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$ontable b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$handempty} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$clear a} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{on b a} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$holding b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\textbf{End} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{clear c} & \multicolumn{1}{l|}{$\neg$clear c} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$ontable c} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$clear b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$ontable b} & \multicolumn{1}{l|}{handempty} & \multicolumn{1}{l|}{$\neg$handempty} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$clear a} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{on b a} & \multicolumn{1}{l|}{on c b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$holding b} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{$\neg$holding c} \\ \hline
\end{tabular}
\end{table}

==> figures/resource_table_3.tex <==
\begin{table*}
\centering
\begin{tabular}{@{}cll@{}}
\toprule
\textit{\textbf{Step}} & \multicolumn{1}{c}{\textit{\textbf{Available Literals}}} & \textit{\textbf{Action}} \\ \midrule

\textbf{Start} & \textbf{clear c}, \textbf{ontable c}, \textbf{clear b}, \textbf{ontable b}, \textbf{handempty}, \textbf{clear a}, \textbf{ontable a} &  \\ \midrule

\textbf{Step 1} & clear c, ontable c, \textbf{clear b}, \textbf{ontable b}, \textbf{handempty}, clear a, ontable a & pick-up \\ \midrule

\textbf{Step 2} & clear c, ontable c, \textbf{holding b}, \textbf{clear a},  $\neg$ontable b,$\neg$clear b, $\neg$handempty, ontable a & stack \\ \midrule

\textbf{Step 3} & \begin{tabular}[c]{@{}l@{}} clear b, \textbf{ clear c}, \textbf{ontable c}, \textbf{handempty}, on b a, $\neg$holding b, $\neg$clear a, $\neg$ontable b, $\neg$clear b, $\neg$handempty, \\ ontable a \end{tabular}& pick-up \\ \midrule

\textbf{Step 4} & \begin{tabular}[c]{@{}l@{}}\textbf{holding c}, \textbf{clear b}, $\neg$ontable c, $\neg$clear c, $\neg$handempty, on b a, $\neg$holding b, $\neg$clear a, $\neg$ontable b, \\ $\neg$clear b, $\neg$handempty, ontable a\end{tabular} & stack \\ \midrule

\textbf{End} & \begin{tabular}[c]{@{}l@{}}clear c, handempty, \textbf{on c b}, $\neg$holding c, $\neg$clear b, $\neg$ontable c$\neg$clear c, $\neg$handempty, \textbf{on b a}, $\neg$holding b, \\ $\neg$clear a, $\neg$ontable b, $\neg$clear b, $\neg$handempty, ontable a\end{tabular} &  \\ \bottomrule
\end{tabular}
\caption{The available literals at every step of the plan can be concluded from the linear notation that encodes the string diagram representation shown in Figure \ref{fig:block_string_diagram}. This can be noticed by reading the diagram from left to right at varying horizontal positions and noting the strings you encounter. The explicitly required literals are colored in \textbf{bold text}. The post-conditions for each action are included as \textit{Available Literals} in the next row.}
\label{table:resources}
\end{table*}
